CLIMATE-FEVER: A Dataset for Verification of Real-World Climate Claims

We introduce CLIMATE-FEVER, a new publicly available dataset for verification of climate change-related claims. By providing a dataset for the research community, we aim to facilitate and encourage work on improving algorithms for retrieving evidential support for climate-specific claims, addressing the underlying language understanding challenges, and ultimately help alleviate the impact of misinformation on climate change. We adapt the methodology of FEVER [1], the largest dataset of artificially designed claims, to real-life claims collected from the Internet. While during this process, we could rely on the expertise of renowned climate scientists, it turned out to be no easy task. We discuss the surprising, subtle complexity of modeling real-world climate-related claims within the \textsc{fever} framework, which we believe provides a valuable challenge for general natural language understanding. We hope that our work will mark the beginning of a new exciting long-term joint effort by the climate science and AI community.

==> 30-evaluation-backup.tex <==
\section{Discussion and future work}


%We collected a total number of 3136 claims concerning climate and climate-change from the internet. These claims were presented to 31 annotators in Task-1 to reject claims that are non-verifiable (see def.~\ref{def:verifiability}). For each claim a total number of 5 votes were to be collected to measure inter-annotator agreement. 

%were only able to collect a complete set of 5 votes for 189 claims. For 2000 claims we collected at least 2 votes. We proceeded to accept all claims with at least 2 votes that have a majority accept vote totaling in 1540 claims. During post-processing we found several examples of claims posed as a question. To keep the dataset compatible with the original FEVER dataset we algorithmically removed these claims. We ended up with a final set of 1535 climate claims (48.9\% of the initially collected claims).

To gain insight into the 1,535 climate claims, we collected several statistics about the dataset. By using a clustering technique, we identified more than 20 different topics represented by the collected claims, such as claims concerning ``climate change in the arctic'', ``sea-level rise'', and more general ones concerning ``climate\_change and global warming'' (see Appendix~\ref{sec:claim-statistics}).

With the annotation process still ongoing, the evidence labelling task (Task-2) produced a dataset of 288 claims with an annotated set of five evidence candidates for each claim.\footnote{The annotation process will be completed in time for the workshop. However, the current preliminary analysis is already representative.} The macro-verdict distribution for labels \texttt{SUPPORTS}, \texttt{REFUTES}, \texttt{CONTRADICTS}, and \texttt{NOT\_ENOUGH\_INFO} is 99 (34.38\%), 42 (14.58\%), 21 (7.29\%), and 126 (43.75\%). We measured an inter-annotator agreement (Krippendorff's alpha) of 0.396 only for claims with a minimum of two votes. For our final \textsc{climate-fever} test-set we reject all contradictory cases, leading to a total number of 267 claims each with a set of five evidence sentences.

Our end-to-end claim-validation pipeline evaluated on the \textsc{climate-fever} test-set yields the following scores: label-accuracy = 47.57\%, recall = 0.48, precision = 0.52, $\mathrm{F}_1$ = 0.41. We computed weighted-averages for the last three metrics to compensate for the unbalanced labels. Again, the real-life nature of the \textsc{climate-fever} dataset proves to be a challenge indicated by the low label-accuracy (47.57\%), as compared to the higher and competitive label-accuracy on the \textsc{fever} test-set (77.68\%). We believe that this result is mainly due to
%is due to two main reasons: First, the \textsc{fever} dataset does only contain a very small subset of claims that are related to climate change. Second, and more importantly, 
the artificial nature of \textsc{fever} claims. As argued above, real-world claims pose some unique challenges and subtleties. For instance, the claim

\texttt{\small ``The melting Greenland ice sheet is already a major contributor to rising sea level and if it was eventually lost entirely, the oceans would rise by six metres around the world, flooding many of the world’s largest cities.'' }

includes a statement that the sea level will rise six meters. An \textsc{ecrs}-retrieved evidence sentence may state a sea level rise of $x+\epsilon$ meters. Although the numbers differ, the climate scientists labelled the evidence as supportive. There are also more demanding cases. For instance, for the claim

\texttt{\small ``An article in Science magazine illustrated that a rise in carbon dioxide did not precede a rise in temperatures, but actually lagged behind temperature rises by 200 to 1000 years.''}

the \textsc{ecrs} provides both supporting and refuting evidence and labelled as such by the annotators. Such contradictory claims are absent in the \textsc{fever} dataset.\footnote{We list more examples of our \textsc{climate-fever} dataset in Appendix \ref{sec:appendix-cf}.} To develop a powerful fact-checking algorithm, we must be able to cope with the complexity of real-life claims in general, and at the same time, account for the specific characteristics of claims related to climate change. With further extending \textsc{climate-fever} and making it publicly available, we provide a first step in the right direction.   %It is intended to give a feeling of the unique challenges and subtleties of real-life claims. 
%In particular it also gives examples of contradictory claims where both supporting and refuting evidence was retrieved by the \textsc{ecrs} and labelled as such by the annotators. We believe that it is important to extend \textsc{fever} with such examples because such claims seem to be a natural phenomenon of real-life statements.

\jbgcomment{I'd really like to see some examples to support your claims.  Talk about how these data are unique and challenging!}

\tdcomment{Add summary of claims + performance on CLIMATE-FEVER dataset (referring appendix B), also mention draw-back of original FEVER dataset not containing contradictory statements which naturally seem to arise for real-life claims.}

==> NeurIPS - Climate Workshop - Thomas Thesis/10-introduction.tex <==
\section{Introduction}\label{sec:Introduction}

With the easy availability of information through the Internet and social media, claims of unknown veracity manipulate public perception and interpretation. %The dissemination of fake news\footnote{We use the term `fake news' to denote information disorders in a broad sense, including misinformation and disinformation.  \jbgcomment{I'd rather focus on an "official" definition with a citation if possible}} can significantly influence political views and discredit authoritative bodies such as government institutions and the scientific community~\cite{lazer2018science}. %Indeed, large-scale and widespread dissemination of fake news threatens the entire political process of democracy, which depends on reliable information.  
Misinformation and disinformation are particularly pressing issues for the climate change debate. They have confused the public, led to political inaction, and stalled support for climate-change mitigation measures~\cite{anderegg2010expert, ding2011support, benegal2018correcting, van2017inoculating}. To counter the influence of potentially false claims on the formation of public opinion on climate change, researchers and experts began to manually assess claims' veracity and publish their assessments on platforms such as \url{climatefeedback.org} and \url{skepticalscience.com}.  

%\jbgcomment{Rather than focusing on fake news, it might be less politically charged to just say that climate change is complicated and hard to understand and people want to understand if claims that they're reading online are supported by sources they trust.}

% Fakenews: https://asistdl.onlinelibrary.wiley.com/doi/full/10.1002/pra2.2015.145052010082

%Recently, new literature on algorithmic fact-checking has emerged, using machine learning and natural language understanding (\textsc{nlu}) to automatically predict the veracity of claims. One of the best-known frameworks on which these efforts are based is \textsc{fever} \cite{thorne2018fever}. It consists of a well-vetted set of %185,445 
%claims and evidence and a common task for evaluating implementations of claim validators. Given that the \textsc{fever} claims are artificially constructed, they may not share the characteristics of real-world claims. Consequently, researchers~\cite{augenstein2019multifc} started to combine real-world claims from multiple fact-checking organizations. However, these databases are constructed for multi-domain veracity prediction and may not be suitable for the topic of climate change. 
%\mccomment{I would focus above primarily on the notion of algorithmically collecting relevant, reliable evidence with respect to a claim. I would avoid giving the impression that we support the idea that machines can be used to automatically predict the veracity of claims. In fact, I would make it clear that this technology can only help provide evidence for humans to make better decisions about these claims' veracity.}


%\mlcomment{Something to include in the intro?\\ https://www.aclweb.org/anthology/2020.lrec-1.849.pdf} 

%We contribute to the literature by adopting the \textsc{fever} framework to collect real-world claims specifically on climate change. We call this database the \textsc{climate-fever} dataset. Making \textsc{climate-fever} publicly available is a crucial first step, enabling the \textsc{nlu} and machine learning communities to develop innovative new fact-checking and verification techniques which could greatly benefit the climate debate.

%\mccomment{Same here. Let's anticipate what the dataset contains, XXXX claims with retrievalk results from Wikipedia where each retrieved snippet is annotated by humans as support/refute/nei.}

Recently, new literature on algorithmic fact-checking has emerged, using machine learning and natural language understanding (\textsc{nlu}) to work on this problem from different angles. One influential framework that combines several of these aspects is \textsc{fever} \cite{thorne2018fever}. It consists of a well-vetted dataset of human-generated claims and evidence retrieved from Wikipedia and a shared-task for evaluating implementations of claim validators. Given that the \textsc{fever} claims are artificially constructed, they may not share the characteristics of real-world claims. Consequently, researchers~\cite{augenstein2019multifc} started to collect real-world claims from multiple fact-checking organizations along with evidence manually curated by human fact-checkers.

We believe that technology cannot and will not in the foreseeable future replace human fact-checkers. But it can help to provide relevant, reliable evidence for humans to make better decisions about the veracity of a claim. In this work, we focus on building a dataset of real-world claims specifically on climate change. We collect 1,535 claims on the Internet. For each claim, we algorithmically retrieve the top five relevant evidence candidate sentences from Wikipedia by the use of \textsc{nlu} where humans annotate each sentence as supporting, refuting, or not giving enough information to validate the claim. We call this database of 7,675 annotated claim-evidence pairs the \textsc{climate-fever} dataset.\footnote{We make this dataset publicly available at \url{http://climatefever.ai}.}.



==> NeurIPS - Climate Workshop - Thomas Thesis/20-approach.tex <==
\section{Methodology}

We adopt a pipeline approach for our evidence retrieval and claim validation system similar to the baseline system proposed by \textsc{fever} \cite{thorne2018fever} and similar to virtually all competing implementations that followed \cite{soleimani2020bert, hanselowski2018ukp, nie2019combining, zhong2019reasoning, liu2020fine}. The reason for building this system is two-fold. First, we require an algorithm to automatically retrieve evidence candidates from a large Knowledge Document Collection\footnote{We define \textsc{kdc} as any large document corpus that contains well-founded textual (prose) representations of knowledge. Examples for \textsc{kdc}'s are encyclopediae, newspaper archives, scientific publications.} (\textsc{kdc}) given a claim to build our dataset. Second, we require an end-to-end claim validation algorithm to predict entailment given a claim and evidence candidates to form a baseline, i.e., to answer the question if current claim validation approaches are up to the task of algorithmically validating real-life claims.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{climateFeverOverviewAlt.jpg}
\caption{\label{fig:pipeline} Overview of the claim validation system consisting of the Evidence Candidate Retrieval System (\textsc{ecrs}) and Entailment Prediction (\textsc{ep}) stage.}
\end{figure}

Our architecture consists of two distinct components, the Evidence Candidate Retrieval System (\textsc{ecrs}) and the Entailment Prediction (\textsc{ep}) stage (see Fig.~\ref{fig:pipeline}). For a given claim, the \textsc{ecrs} retrieves sentences as evidence candidates from the \textsc{kdc}. A pair of claim and evidence candidate sentences are fed to the \textsc{ep} to predict one of the labels \texttt{SUPPORTS}, \texttt{REFUTES} or \texttt{NOT\_ENOUGH\_INFO}, depending on whether the evidence is supporting, refuting, or not giving enough information to validate the given claim. The \textsc{fever} dataset uses a copy of the English Wikipedia containing only the introductory section of all articles as \textsc{kdc}. We also use the English Wikipedia as \textsc{kdc} but, given the complexity of real-life climate claims, allow the complete body of Wikipedia articles as a source of evidence.\footnote{This extension introduces a challenge with respect to the retrieval of evidence candidates. In the original setup, the number of sentences retrieved after the document retrieval stage is permitting for pairwise ranking against a given claim (up to 100 sentences on average in the introductory section). In our case, the number of sentences becomes intractable. We, therefore, introduce a novel technique by leveraging learned sentence-embeddings combined with a fast vector similarity index, \textsc{faiss} \cite{JDH17}, to pre-select the most relevant sentences given a claim prior to the pairwise re-ranking. This can be compared to Facebook AI's Dense Passage Retrieval (\textsc{dpr}) \cite{karpukhin2020dense} that uses a similar approach for solving Open-Domain Question Answering (\textsc{qa}) by using dense embeddings rather than BM25.
} 

\subsection{Retrieving and labeling climate claims (Task-1)}

%We devised an \foreign{ad hoc} approach to collect climate claims from the Internet. By using a set of seed keywords (climate, climate change, climate hoax, global warming, etc.), several Google searches were performed to find possible sources for such claims. The claims were then either manually retrieved or the pages were automatically scrapped using Python packages (\texttt{requests}\footnote{An elegant Python library for HTTP requests, \url{https://requests.readthedocs.io/en/master/}.}, \texttt{BeautifulSoup}\footnote{A Python library for extracting data out of (noisy) HTML/XML files, \url{https://www.crummy.com/software/BeautifulSoup/bs4/doc/}.}).
%As a minimal goal, at least 1000 claims were to be collected to form a dataset large enough for quantitative evaluation. We require a balanced set of claims with respect to scientific consensus, i.e., one half of the \textsc{climate-fever} claims should be collected from scientifically sound sources while the other half should be collected from known climate change denial sources.
%The variability in quality of the collected claims, i.e.,  in terms of fluency, was quite large. Therefore, for producing a high-quality dataset, the claims needed to be manually vetted. We prepared an annotation process that allowed human annotators to label the claims with respect to the notion of verifiability, as defined in the next section. For both our annotation tasks we used the Prodigy annotation framework\footnote{Prodigy is a proprietary annotation tool for data labelling tasks, \url{https://prodi.gy/}.}.

%\jbgcomment{How did you use Google searches?  Some API?}

To obtain a set of candidate climate claims from the Internet, we follow an \foreign{ad-hoc} approach and use a set of seed keywords in Google searches\footnote{For this study we did not automate this step. Instead, we manually searched for seed keywords, identified potential targets, and used Python libraries such as \texttt{requests} and \texttt{BeautifulSoup} to download, parse and clean content for subsequent processing.} to identify possible sources for such claims. We either retrieved the claims manually, or we scraped the pages automatically. We collected an equal number of \textsc{climate-fever} claims from both scientifically-informed and climate change skeptics/deniers sources. This procedure resulted in a balanced set of more than 3,000 climate claims. %Given the high variability in the quality of the collected claims, we further vetted the claims to obtain a high-quality dataset manually. 
%\tdcomment{I changed it accordingly.}

\textsc{fever} claims were written and curated by annotators, enforcing a rigorous set of requirements for writing claims. The resulting claims are self-contained, short, and syntactically simple. For example, one of the rare claims related to climate change in \textsc{fever} reads: 

\texttt{\small "The Gray wolf is threatened by global warming."} 

In contrast, a candidate claim crawled from the wild is, e.g.:

\texttt{\small ``The Intergovernmental Panel on Climate Change is misleading humanity about climate change and sea levels, and that in fact, a new solar-driven cooling period is not far off.''}

Given the complexity of real claims, we introduce the definition of a verifiable claim as follows.


%We resolve the lacuna by introducing the notion of verifiable claims. 



%\mlcomment{Can we say somewhere that our analysis provides empirical support for the need for a dataset with real claims?}
%\mlcomment{Can we maybe extract a climate-related claim from FEVER and one from our database to see the material difference between the two?}




%Therefore, we designed an annotation process in which human annotators labeled the claims with respect to the notion of verifiability, which we define below.
\begin{definition}[Verifiable claims]
\label{def:verifiability}
A claim is potentially \emph{verifiable} if it is a) well-formed and b) subjectively investigable. 
\begin{itemize*}
    \item[a)]\label{def:wellformed} A \emph{well-formed} claim is a single English sentence, consistent, unambiguous, and complete (i.e., not much implicit knowledge is needed for comprehension by the reader). 
    \item[b)]\label{def:investigable} A claim is \emph{subjectively investigable}, if evidence could be retrieved from a knowledge document collection (\textsc{kdc}) that decreases the investigators uncertainty about the truthfulness (or falsehood) of the statement.
\end{itemize*}
\end{definition}
Equipped with our definition of verifiable claims, we asked climate scientists to label our collected claims (Task 1). For each claim, we collected up to five votes. This annotation task resulted in more than 1,535 verifiable climate claims on which there was a sufficient consensus among the annotators. We give examples of verifiable and non-verifiable claims in Appendix \ref{sec:appendix-task-1}.

%\jbgcomment{It's not clear that this is a contribution (it is!).  This needs to be worded to say something like: existing definitions fail for reasons X,Y,Z.  We resolve this lacuna by A,B,C.}

\subsection{Evidence candidate retrieval}

%Manually searching for and finding sentences as evidence candidates in a large \textsc{kdc}, such as Wikipedia, for several hundreds of claims is infeasible. To address this problem, 
To automatically retrieve relevant evidence candidates from Wikipedia for a given claim, we build an \textsc{ecrs} pipeline consisting of the following three steps\footnote{For BM25 in the first step we leverage Apache's Lucene (\url{https://lucene.apache.org/}), while our model implementations for steps two and three are both based on Google's \textsc{albert} model \cite{lan2019albert} by using HuggingFace's \texttt{transformers} library \cite{Wolf2019HuggingFacesTS}.}:
%
%\begin{enumerate*}
%    \item \emph{Document-Level Retrieval}: Given a claim as input, retrieve the most relevant documents from the \textsc{kdc}. We apply an entity-linking approach similar to \cite{hanselowski2018ukp}. We use BM25 \cite{robertson2009probabilistic} to query an inverse document index containing all English Wikipedia articles with entity mentions extracted from the claim. We use a dependency parser to identify candidates of entity mentions, i.e., by extracting noun-phrases. We select the top-10 relevant articles.
%    \item \emph{Sentence-Level Retrieval}: Given a claim as input, retrieve the most relevant sentences from the documents selected by the previous step. We introduce sentence-embeddings trained on the \textsc{fever} dataset to capture finer-grained semantic similarities between a claim and evidence sentences. We measure similarity by computing the $L^2$ distance between normalized sentence vectors of claim and evidence sentences (this is equivalent to computing the cosine distance between the vectors). We select the top-100 relevant sentences. To produce task-specific sentence-embeddings, we adopt a pretrained \textsc{albert} (large-v2) model in an average-pooled Siamese-setting \cite{reimers2019sentence} trained with a triplet-loss objective on triplets of (claim, relevant evidence, negative evidence). We apply hard positive and negative mining \cite{hermans2017defense,soleimani2020bert} to compensate for the large number of possible negative examples. For each claim we create one batch of fixed size of which up to one half of evidence sentences are positive examples (i.e., supporting or refuting evidence given the evidence sentence), and the rest is filled with randomly sampled sentences from the \textsc{fever} Wikipedia dump to form the set of negative evidence sentences. After the forward-pass through the model, we select the hardest positive and the hardest negative pair to form the triplet for optimization. We train until convergence.
%    \item \emph{Sentence Re-Ranking}: Finally, we re-rank the retrieved sentences from the previous steps given the input claim to find the top 5 most relevant candidates. Similar to \cite{soleimani2020bert} we train a point-wise model to predict a relevance score for pairs of claim and evidence. To compensate for missing co-reference pronouns in the evidence sentences, we prepend the Wikipedia pages titles to each evidence candidate. We adopt a pretrained \textsc{albert} (base-v2) model with a binary classifier on the \texttt{[CLS]} token. Every evidence is classified as \emph{evidence} (1) or \emph{non-evidence} (0). During training, we use claims along with supporting and refuting evidence from the \textsc{fever} training split as examples for \emph{evidence} and we randomly sample sentences from the \textsc{fever} Wikipedia dump to provide examples for \emph{non-evidence}. During inference, we sort evidence sentences by the predicted output in descending order and take the top-5 sentences. 
%\end{enumerate*}

\emph{1. Document-level retrieval}: Given a claim as input, we retrieve the most relevant documents from the \textsc{kdc}. We apply an entity-linking approach similar to \cite{hanselowski2018ukp}. We use BM25 \cite{robertson2009probabilistic} to query an inverse document index containing all English Wikipedia articles with entity mentions extracted from the claim. We use a dependency parser to identify candidates of entity mentions, and we select the top-10 relevant articles.

\emph{2. Sentence-level retrieval}: From the selected articles, we retrieve the top-100 most relevant sentences using sentence-embeddings trained on the \textsc{fever} dataset. % to capture finer-grained semantic similarities between a claim and evidence sentences. %We measure similarity by computing the $L^2$ distance between normalized sentence vectors of claim and evidence sentences (this is equivalent to computing the cosine distance between the vectors). 
To produce task-specific sentence-embeddings, we adopt a pretrained \textsc{albert} (large-v2) model in an average-pooled Siamese-setting \cite{reimers2019sentence}. %trained with a triplet-loss objective on triplets of (claim, relevant evidence, negative evidence). 
We apply hard positive and negative mining \cite{hermans2017defense,soleimani2020bert} to compensate for the large number of possible negative examples. %For each claim we create one batch of fixed size of which up to one half of evidence sentences are positive examples (i.e. supporting or refuting evidence given the evidence sentence) and the rest is filled with randomly sampled sentences from the \textsc{fever} Wikipedia dump to form the set of negative evidence sentences. After the forward-pass through the model, we select the hardest positive and the hardest negative pair to form the triplet for optimization. We train until convergence.

\emph{3. Sentence re-ranking}: %We re-rank the retrieved sentences from the previous step, given the input claim to find the top 5 most relevant candidates. 
Similar to \cite{soleimani2020bert} we train a point-wise model to predict a relevance score for pairs of claim and evidence. 
%To compensate for missing co-reference pronouns in the evidence sentences, we prepend the Wikipedia pages titles to each evidence candidate. 
We adopt a pretrained \textsc{albert} (base-v2) model with a binary classifier on the \texttt{[CLS]} token. Every evidence is classified as \emph{evidence} (1) or \emph{non-evidence} (0). During training, we use claims along with supporting and refuting evidence from the \textsc{fever} training split as examples for \emph{evidence} and we randomly sample sentences from the \textsc{fever} Wikipedia dump to provide examples for \emph{non-evidence}. During inference, we sort evidence sentences by the predicted score in descending order and select the top five sentences.

%\jbgcomment{These steps can likely be trimmed.  Cite methods from other papers when you can, summarize where you can't.}

\subsection{Evidence candidate labelling (Task-2)}

%%In Task-2, the claims together with their five evidence sentences as retrieved by the \textsc{ecrs} are displayed to the annotators to label it as \emph{supporting}, \emph{refuting}, or \emph{not giving enough information to validate} the claim.\footnote{Given our 1,535 climate claims and five sentences per claim, we end up with 7,675 annotations.} %We split the 7675 tasks into 10 slices, each containing 770 claim-evidence pairs (745 pairs for the last slice). 
%%For each claim, we collect five individual votes per claim-evidence pair, which allows us to analyze confidence and to compute inter-annotator agreement. 
%%During post-processing we compute a micro-verdict (for every claim-evidence pair) and a macro-verdict (aggregated verdict for every claim). The micro-verdict is given by the majority-vote for each claim-evidence pair. % (i.e. micro-verdict \texttt{SUPPORTS} for 3 votes \texttt{SUPPORTS}, 1 vote \texttt{REFUTES}, 1 vote \texttt{NOT\_ENOUGH\_INFO}. 
%%For the macro-verdict, we aggregate the micro-verdicts of all five evidences for each claim. %\footnote{The macro-verdict is \texttt{SUPPORTS}, if at least one micro-verdict is \texttt{SUPPORTS} and all others are \texttt{NOT\_ENOUGH\_INFO}; it is \texttt{REFUTES}, if at least one micro-verdict is \texttt{REFUTES} and all others are \texttt{NOT\_ENOUGH\_INFO}; it is \texttt{NOT\_ENOUGH\_INFO}, if all micro-verdicts are \texttt{NOT\_ENOUGH\_INFO}; otherwise the macro-verdict is \texttt{CONTRADICTS}.}

In Task-2, the claims together with their top five evidence sentences as retrieved by the \textsc{ecrs} are displayed to the annotators to label it as \emph{supporting}, \emph{refuting}, or \emph{not giving enough information to validate} the claim.\footnote{Given our 1,535 climate claims and five sentences per claim, we end up with 7,675 annotations.} For each claim, we collect five individual votes per claim-evidence pair, which allows us to analyze confidence and to compute inter-annotator agreement.
During post-processing we compute a micro-verdict (for every claim-evidence pair) and a macro-label for every claim (aggregated on the five micro-verdicts). The micro-verdict is given by the majority-vote for each claim-evidence pair (or it is \texttt{NOT\_ENOUGH\_INFO} on a tie). The claim-label is by default \texttt{NOT\_ENOUGH\_INFO} unless there is supporting (\texttt{SUPPORTS}) \emph{or} refuting (\texttt{REFUTES}) evidence. If there is both supporting \emph{and} refuting evidence the claim-label is \texttt{DISPUTED}.


% “Ice berg melts, ocean level remains the same.”
%?? [wiki/Ice_shelf] “The melting of floating ice raises the ocean level". 
%Supports [wiki/Antarctica] “This ice is formed from the ocean water and floats in the same water and thus does not contribute to rise in sea level.”
%Both evidence statements are true in a sense. The first one refers to a rise of only 4 cm if all floating ice shelves were to melt, but this information is missing from the sentence (Noerdlinger & Brower, 2007). What is the correct verdict? Expert knowledge is required to give the right answer.

\subsection{Entailment prediction}

For entailment prediction, the top five candidate evidence sentences along with the corresponding Wikipedia article titles are jointly compared against the claim to predict one of the labels \texttt{SUPPORTS}, \texttt{REFUTES}, or \texttt{NOT\_ENOUGH\_INFO}. We adopt a pretrained \textsc{albert} (large-v2) with a three-way classifier on the \texttt{[CLS]} token of a concatenation of claim and evidence sentences\nothing{Pairs of (article title, evidence sentence) are concatenated, i.e. ``Title-1: Sentence-1. Title-2: Sentence-2, \ldots, Title-5: Sentence-5.'', and then encoded to form one input sequence to the \textsc{albert} tokenizer while the other input sequence being the encoded claim.}. We train the model by using the \textsc{ecrs} to retrieve the top five evidence candidates for each claim from the \textsc{fever} training split and use the gold-labels as ground-truth for optimizing the cross-entropy loss. We reach a competitive label-accuracy of 77.68\% on the \textsc{fever} dev-set using our end-to-end pipeline (\textsc{sota} label-accuracy of 79.16\% on the dev-set is reported by \cite{zhong2019reasoning}). For measuring the end-to-end performance of our claim-validation pipeline on the \textsc{climate-fever} dataset, we predict labels for all claim and evidence-set pairs and compare against the gold-labels (claim-labels) from Task-2.



==> NeurIPS - Climate Workshop - Thomas Thesis/30-evaluation-backup.tex <==
\section{Discussion and future work}


%We collected a total number of 3136 claims concerning climate and climate-change from the internet. These claims were presented to 31 annotators in Task-1 to reject claims that are non-verifiable (see def.~\ref{def:verifiability}). For each claim a total number of 5 votes were to be collected to measure inter-annotator agreement. 

%were only able to collect a complete set of 5 votes for 189 claims. For 2000 claims we collected at least 2 votes. We proceeded to accept all claims with at least 2 votes that have a majority accept vote totaling in 1540 claims. During post-processing we found several examples of claims posed as a question. To keep the dataset compatible with the original FEVER dataset we algorithmically removed these claims. We ended up with a final set of 1535 climate claims (48.9\% of the initially collected claims).

To gain insight into the 1,535 climate claims, we collected several statistics about the dataset. By using a clustering technique, we identified more than 20 different topics represented by the collected claims, such as claims concerning ``climate change in the arctic'', ``sea-level rise'', and more general ones concerning ``climate\_change and global warming'' (see Appendix~\ref{sec:claim-statistics}).

With the annotation process still ongoing, the evidence labelling task (Task-2) produced a dataset of 288 claims with an annotated set of five evidence candidates for each claim.\footnote{The annotation process will be completed in time for the workshop. However, the current preliminary analysis is already representative.} The macro-verdict distribution for labels \texttt{SUPPORTS}, \texttt{REFUTES}, \texttt{CONTRADICTS}, and \texttt{NOT\_ENOUGH\_INFO} is 99 (34.38\%), 42 (14.58\%), 21 (7.29\%), and 126 (43.75\%). We measured an inter-annotator agreement (Krippendorff's alpha) of 0.396 only for claims with a minimum of two votes. For our final \textsc{climate-fever} test-set we reject all contradictory cases, leading to a total number of 267 claims each with a set of five evidence sentences.

Our end-to-end claim-validation pipeline evaluated on the \textsc{climate-fever} test-set yields the following scores: label-accuracy = 47.57\%, recall = 0.48, precision = 0.52, $\mathrm{F}_1$ = 0.41. We computed weighted-averages for the last three metrics to compensate for the unbalanced labels. Again, the real-life nature of the \textsc{climate-fever} dataset proves to be a challenge indicated by the low label-accuracy (47.57\%), as compared to the higher and competitive label-accuracy on the \textsc{fever} test-set (77.68\%). We believe that this result is mainly due to
%is due to two main reasons: First, the \textsc{fever} dataset does only contain a very small subset of claims that are related to climate change. Second, and more importantly, 
the artificial nature of \textsc{fever} claims. As argued above, real-world claims pose some unique challenges and subtleties. For instance, the claim

\texttt{\small ``The melting Greenland ice sheet is already a major contributor to rising sea level and if it was eventually lost entirely, the oceans would rise by six metres around the world, flooding many of the world’s largest cities.'' }

includes a statement that the sea level will rise six meters. An \textsc{ecrs}-retrieved evidence sentence may state a sea level rise of $x+\epsilon$ meters. Although the numbers differ, the climate scientists labelled the evidence as supportive. There are also more demanding cases. For instance, for the claim

\texttt{\small ``An article in Science magazine illustrated that a rise in carbon dioxide did not precede a rise in temperatures, but actually lagged behind temperature rises by 200 to 1000 years.''}

the \textsc{ecrs} provides both supporting and refuting evidence and labelled as such by the annotators. Such contradictory claims are absent in the \textsc{fever} dataset.\footnote{We list more examples of our \textsc{climate-fever} dataset in Appendix \ref{sec:appendix-cf}.} To develop a powerful fact-checking algorithm, we must be able to cope with the complexity of real-life claims in general, and at the same time, account for the specific characteristics of claims related to climate change. With further extending \textsc{climate-fever} and making it publicly available, we provide a first step in the right direction.   %It is intended to give a feeling of the unique challenges and subtleties of real-life claims. 
%In particular it also gives examples of contradictory claims where both supporting and refuting evidence was retrieved by the \textsc{ecrs} and labelled as such by the annotators. We believe that it is important to extend \textsc{fever} with such examples because such claims seem to be a natural phenomenon of real-life statements.

\jbgcomment{I'd really like to see some examples to support your claims.  Talk about how these data are unique and challenging!}

\tdcomment{Add summary of claims + performance on CLIMATE-FEVER dataset (referring appendix B), also mention draw-back of original FEVER dataset not containing contradictory statements which naturally seem to arise for real-life claims.}

==> NeurIPS - Climate Workshop - Thomas Thesis/30-evaluation.tex <==
\section{Discussion and future work}

To gain insight into the 1,535 climate claims, we collected several statistics about the dataset. By using a clustering technique, we identified more than 20 different topics represented by the collected claims, such as claims concerning ``climate change in the arctic'', ``sea-level rise'', and more general ones concerning ``climate\_change and global warming'' (see Appendix~\ref{sec:claim-statistics}).

The evidence labelling task (Task-2) produced a dataset of 1,535 claims with an annotated set of five evidence candidates for each claim. Each evidence sentence is labelled by at least two voters ($\num{2.4 \pm 0.7}$ voters per evidence on average). The distribution for aggregate claim-labels \texttt{SUPPORTS}, \texttt{REFUTES}, \texttt{DISPUTED}, and \texttt{NOT\_ENOUGH\_INFO} is 655 (42.67\%), 253 (16.5\%), 153 (9.97\%), and 474 (30.88\%). While \textsc{fever} only contains undisputed claims, we include claims for which both supporting and refuting evidence were found. We believe that these examples are especially useful since they appear to be a common feature of real-world claims.

Furthermore, we dealt with the limitation of \textsc{fever}-style majority-vote based aggregation for deciding on a claim label. The approach is too naïve as, in many cases, retrieved evidence covers only some facets of the claim, in which case not enough evidence is present to form a final opinion. More generally, a claim (hypothesis) can at best be refuted by contrarian evidence. Epistemologically, it is impossible to assign a final verdict. In our case, the only purpose for assigning a gold-label to each climate-claim is to measure a baseline performance of a \textsc{fever} entailment predictor on our dataset. Our dataset provides both the micro-verdict labels and the claim-labels for each claim-evidence pair.

For Task-2 we measured an average inter-annotator agreement (Krippendorff's alpha) of 0.334. This low level of agreement signifies the hardness of the task, i.e., even for human annotators, it is non-trivial to decide if an evidence candidate supports or refutes a given claim. Table~\ref{tab:disagreement-overviews} details the level of disagreement on a per-slice basis.\footnote{For Task-2 we split the 1,535 claims into 10 slices of 770 claims each (except for the last slice) such that each annotator has to label 3,850 claim-evidence pairs.} We observed that training the annotators can help raise the agreement level (e.g.\ slice 8 was labelled by two second-time annotators). Furthermore, we could also see that pairs of annotators that are experts on the topic (e.g.,  climate scientists or ML specialists) tend to have a higher average agreement (cf.\ slices 0 and 3).

\begin{table}[t]
	\centering
	\caption{\label{tab:disagreement-overviews} For evidence candidate labelling (Task-2) the 1,535 claims were split into 10 slices of 770 claims each (except for the last slice). Each slice consists of 3,850 ($770 \times 5$) claim-evidence pairs. This table lists for each slice the average number of voters, the inter-annotator agreement ($\alpha_\mathrm{Krippendorff}$), the fraction of evidence sentences with total agreement and the average entropy with respect to the select class (\texttt{SUPPORTS}, \texttt{REFUTES} or \texttt{NOT\_ENOUGH\_INFO}).}
	\begin{tabular}{rrrrrr}
		\toprule
		Slice &  Size &  Avg.\ Num.\ Voters &  $\alpha_\mathrm{Krippendorff}$ &  Total Agreement &  Avg.\ Entropy \\
		\midrule
		0 &   770 &             2.227 &  0.283 &            \textbf{0.613} &         0.266 \\
		1 &   770 &             4.019 &  0.399 &            0.423 &         0.380 \\
		2 &   770 &             2.000 &  0.522 &            \textbf{0.745} &         0.176 \\
		3 &   770 &             3.001 &  0.106 &            0.201 &         0.544 \\
		4 &   770 &             2.000 &  0.215 &            0.504 &         0.344 \\
		5 &   770 &             2.000 &  0.091 &            0.404 &         0.413 \\
		6 &   770 &             2.000 &  0.252 &            0.529 &         0.327 \\
		7 &   770 &             2.825 &  0.316 &            0.461 &         0.371 \\
		8 &   770 &             2.000 &  0.431 &            \textbf{0.635} &         0.253 \\
		9 &   745 &             2.000 &  0.229 &            0.545 &         0.315 \\
		\bottomrule
	\end{tabular}
\end{table}


The \textsc{fever}-trained entailment-predictor evaluated on the \textsc{climate-fever} dataset\footnote{To stay compatible with the \textsc{fever} methodology for evaluation we simply excluded disputed claims from our dataset.} yields the following scores (cf.\ table \ref{tab:classification-report}): label-accuracy = 38.78\%, recall = 38.78\%, precision = 56.49\%, $\mathrm{F}_1$ = 32.85\%. We computed weighted-averages for the last three metrics to compensate for the unbalanced labels. The real-life nature of the \textsc{climate-fever} dataset proves to be a challenge indicated by the low label-accuracy (38.78\% --- only slightly better than chance classification), as compared to the higher and competitive label-accuracy on the original \textsc{fever} dev-set (77.69\%). As can be seen in table \ref{confusion-matrix}, the model particularly struggles to predict \texttt{SUPPORTED} claims while it performs slightly better on predicting \texttt{REFUTED} claims. We suspect that this result can mainly be attributed to the stark qualitative differences between real-world claims of \textsc{climate-fever} and the artificial nature of \textsc{fever} claims. As argued above, real-world claims pose some unique challenges and subtleties. For instance, the claim

\texttt{\small ``The melting Greenland ice sheet is already a major contributor to rising sea level and if it was eventually lost entirely, the oceans would rise by six metres around the world, flooding many of the world’s largest cities.'' }

includes a statement that the sea level will rise six meters. An \textsc{ecrs}-retrieved evidence sentence may state a sea-level rise of $x+\epsilon$ meters. Although the numbers differ, the climate scientists labelled the evidence as supportive. There are also more demanding cases. For instance, for the claim

\texttt{\small ``An article in Science magazine illustrated that a rise in carbon dioxide did not precede a rise in temperatures, but actually lagged behind temperature rises by 200 to 1000 years.''}

the \textsc{ecrs} provides both supporting and refuting evidence and labelled as such by the annotators. Such disputed claims are absent in the \textsc{fever} dataset.\footnote{We list more examples of our \textsc{climate-fever} dataset in Appendix \ref{sec:appendix-cf}.} To develop new strategies for tackling (climate-related) disinformation, we must be able to cope with the complexity of real-life claims in general, and at the same time, account for the specific characteristics of claims related to climate change. By further extending \textsc{climate-fever} and making it publicly available, we provide a first step in the right direction and hope that our work will stimulate a new long-term joint effort by climate science and \textsc{ai} community.

% limitations: Annotations were done on individual evidence level. Macro-verdict is computed by aggregating micro-verdicts on individual evidence candidates. One should do another pass where meta-labellers are deciding the macro-label based on the labelled evidence sentences.


==> NeurIPS - Climate Workshop - Thomas Thesis/ack.tex <==
\section*{Acknowledgments}
%We would like to thank Thomas Hofmann, Reto Knutti, ... more names of people that have contributed and maybe one generic way of thanking all the others who have contributed annotations...

We would like to thank Thomas Hofmann (ETH Zurich) for his helpful contribution to an early draft of this paper. We also thank Christian Huggel (University of Zurich) and Reto Knutti (ETH Zurich) for all their comments and their climate science expertise. Finally, we are grateful to all climate scientists and annotators who were involved in the annotation process to build the \textsc{climate-fever} database. Research supported with Cloud \textsc{tpu}s from Google's TensorFlow Research Cloud (\textsc{tfrc}).

%for his viable expertise on climate science. We would like to extend our gratitude to Christian Huggel (University of Zurich) for connecting us to the EClim research group and for introducing us to the International Universities Climate Alliance. We thank \texttt{explosion.ai} for providing us with a complimentary academic licence of the annotation tool that we used for collecting annotations. Finally, we would like to thank all annotators that helped us to make \textsc{climate-fever} possible.

==> NeurIPS - Climate Workshop - Thomas Thesis/conclusion.tex <==
\section{Conclusion}

==> conclusion.tex <==
\section{Conclusion}
